Unified Multi-Domain Learning and Data Imputation using Adversarial Autoencoder

We present a novel framework that can combine multi-domain learning (MDL), data imputation (DI) and multi-task learning (MTL) to improve performance for classification and regression tasks in different domains. The core of our method is an adversarial autoencoder that can: (1) learn to produce domain-invariant embeddings to reduce the difference between domains; (2) learn the data distribution for each domain and correctly perform data imputation on missing data. For MDL, we use the Maximum Mean Discrepancy (MMD) measure to align the domain distributions. For DI, we use an adversarial approach where a generator fill in information for missing data and a discriminator tries to distinguish between real and imputed values. Finally, using the universal feature representation in the embeddings, we train a classifier using MTL that given input from any domain, can predict labels for all domains. We demonstrate the superior performance of our approach compared to other state-of-art methods in three distinct settings, DG-DI in image recognition with unstructured data, MTL-DI in grade estimation with structured data and MDMTL-DI in a selection process using mixed data.

==> parking.tex <==
% %-------------
% \subsection{Selection Process}
% %-------------
% We also evaluate our method in a real world problem that contains structure data with features containing continuous and categorical values. In this setting, our data comes from 3 different companies that use selection processes with a similar structure. For privacy requirements, we refer to the companies with indexes, such that $C_1$ refers to Company 1. 

% $C_1$ is an organization that selects students to receive fellowships. $C_2$, is a big retail company that select students to work in the company after graduation. $C_3$ is a governmental agency that selects students for public administration positions. Table~\ref{tab:process} presents the description for each stage in in each process.

% Each dataset contains sub-datasets. For example, in $C_1$, the process happens annually and we have data for three years, $year_1^{C1}$, $year_2^{C1}$, $year_3^{C1}$. The process in $C_2$ happens every semester and data for 6 semesters is available. The process in $C_3$ also happens annually and 2 years of data are available. In order to adequate the processes, we combine data for two consecutive semesters in $C_2$ to form datasets per year, keeping the last information in case of duplicated applicants. We also use data from the two years available in $C_3$, which overlap with available data from $C_1$ and $C_2$.

% Each stage in the process contains its own set of variables. For example, in the stage \textit{Demographics}, information about state and city is collected. Therefore, we refer to \textit{Demographics} features for those collected in the \textit{Demographics} stage. The data collected in each process is very similar in stages such as \textit{Demographics} and \textit{Education}, both in the form of content and structure. For stages with open questions such as \textit{Video}, each process has its own specific questions.
% \input{tables/process.tex}
% %-------------------------------------------------------------
% \subsubsection{Feature preparation for tabular data}
% %-------------------------------------------------------------
% Categorical variables are converted to numerical values using a standard one-hot encode transformation. In the later stages, such as video, the speech is extracted and the data is used as a text. To convert this data to numerical values, we create word embeddings using Word2Vec~\cite{mikolov2013efficient}, where we assign high-dimensional vectors (embeddings) to words in a text corpus but preserving their syntactic and semantic relationships.
% % %-------------------------------------------------------------
% \subsubsection{Validation and performance metrics for selection}
% %-------------------------------------------------------------
% Our goal for each process is to predict which applicants will be selected in the \textit{Video Evaluation} stage. As seen in Table~\ref{tab:process}, the sample size for each dataset is relatively small which causes classifiers to overfit when trained individually. Although the real evaluation in each process happens independently and the goals are distinct, we believe we can use the datasets together due to the similar structure of the features and the common focus on undergraduate students in their last year. 
 
% We perform longitudinal experiments, in which we use a previous year as a training and test set and the following year as a validation set. For $C_1$ for example, we split the dataset from $year_1^{C1}$ in train and test, find the best model and validate its results using the dataset from $year_2^{C1}$. The model is trained in $year_1^{C1}$ and has never seen any data in $year_2^{C1}$. 

% We also perform experiments in the standard cross-validation setting by using data from a specific year and splitting it in train, test and validation. We repeat this process 3 times, one for each year and one for a dataset with both years combined.

% We use 10-fold cross validation in each experiment with a total of 80 runs. In all experiments, we compare the models in terms of F1-score for the positive class, which balances precision and recall specific for the selected applicants.

% To the best of our knowledge, this is the first approach to directly tackle DG and DI in the same framework. We also focus on the aggregation of smaller labelled datasets to achieve better classification scores for each domain. Therefore, for the selection process case, we validate the methods by: (1) using all datasets as seen source domains with their labels; (2) we aim to find the best classifier, individual for each domain or general for all domains. 
